Unraveling the Viral Spread of Misinformation: Maximum-Likelihood Estimation and Starlike Tree Approximation in Markovian Spreading Models

Identifying the source of epidemic-like spread in networks is crucial for removing internet viruses or finding the source of rumors in online social networks. The challenge lies in tracing the source from a snapshot observation of infected nodes. How do we accurately pinpoint the source? Utilizing snapshot data, we apply a probabilistic approach, focusing on the graph boundary and the observed time, to detect sources via an effective maximum likelihood algorithm. A novel starlike tree approximation extends applicability to general graphs, demonstrating versatility. Unlike previous works that rely heavily on structural properties alone, our method also incorporates temporal data for more precise source detection. We highlight the utility of the Gamma function for analyzing the ratio of the likelihood being the source between nodes asymptotically. Comprehensive evaluations confirm algorithmic effectiveness in diverse network scenarios, advancing source detection in large-scale network analysis and information dissemination strategies.

==> experiments.tex <==
\section{Experiments}\label{sec:sim}


This section first provides numerical examples to illustrate the properties of the proposed estimator on starlike trees; then we compare the starlike tree approximation with existing methods in different networks.

\subsection{Starlike tree graphs}

To demonstrate the capability of simplification of the starlike tree approximation in Algo. \ref{alg:star_contract}, we first list out the closed form of the estimator $\Tilde{P}(G_{\text{N}}|v, T)$ and the likelihood $P(G_{\text{N}}|v, T)$ for different starlike trees in Tab. \ref{tab:closeform_line_end}. We then plot the estimator $\Tilde{P}(G_{\text{N}}|v, T)$ numerically in Fig. \ref{fig:line-graph-leaf-infected} and \ref{fig:ML_star_graph_B3}. From Tab. \ref{tab:closeform_line_end}, we can observe that when $G$ is a line graph (a starlike tree with two arms), we have $P(G_{\text{N}}|v, T)=\Tilde{P}(G_{\text{N}}|v, T)$ for all $v\in G_N$.  If $G$ has more than two arms and $v$ is the central node of the starlike tree, then we still have $P(G_{\text{N}}|v, T)=\Tilde{P}(G_{\text{N}}|v, T)$. Otherwise, the approximation $\Tilde{P}(G_{\text{N}}|v, T)$ serves as a lower bound of $P(G_{\text{N}}|v, T)$ which justify the results in Lemma \ref{lemma:independen}.

\begin{table}[h]
\centering
\small\addtolength{\tabcolsep}{-5pt}

\begin{tabular}{|c|c|c|c|}
\hline
Fig. & $v$ & $\Tilde{P}(G_{\text{N}}|v, T)$ & $P(G_{\text{N}}|v, T)$ \\ \hline
\multirow{2}{*}{5(a)} & $v_0$ & $\frac{1}{2}T^2e^{-T}$   &  $\frac{1}{2}T^2e^{-T}$  \\ \cline{2-4} 
                      & $v_1$ & $T(1-e^{-T})e^{-T}$      &  $T(1-e^{-T})e^{-T}$ \\ \hline
\multirow{2}{*}{6(a)} &$v_0$  & $T^3e^{-3T}$             &  $T^3e^{-3T}$ \\ \cline{2-4} 
                      &  $v_1$  & $\frac{1}{4}T^4e^{-3T}$ & $(2e^T-T^2-2T-2)e^{-3T}$ \\ \hline
%\multirow{2}{*}{6(a)} &$v_0$  &  $T^4e^{-4T}$  &  $T^4e^{-4T}$\\ \cline{2-4} 
%                  & $v_1$ & $\frac{1}{8}T^6e^{-4T}$   & $\frac{1}{8}(3e^{2T}-4T^3-6T^2-6T-3)e^{-4T}$ \\ \hline
\end{tabular}
    \caption{Comparison between the true likelihood $P(G_{\text{N}}|v, T)$ and its approximation $\Tilde{P}(G_{\text{N}}|v, T)$, when considering starlike graphs shown in Fig. \ref{fig:line-graph-leaf-infected} and \ref{fig:ML_star_graph_B3}.}
    \label{tab:closeform_line_end}
\end{table}



Next, we consider the case of different starlike trees $G_N$ containing a leaf node of $G$. In Fig. \ref{fig:line-graph-leaf-infected} and \ref{fig:ML_star_graph_B3}, a node that is colored in white represents uninfected nodes. Otherwise, it is infected. In the scenario where exactly one leaf node of a line graph is infected, \figref{fig:line-graph-leaf-infected} presents the maximum likelihood probability versus spreading time for each node to be the source, as approximated by the starlike tree method. The node with the highest likelihood probability over time is identified as the detected source. 
In each line graph in ~\figref{fig:line-graph-leaf-infected}, node $0$ is an infected leaf node of the underlying network $G$, and node $i$ is connected to node $(i-1)$ for $i\geq 1$. If there are 1 or 2 infected nodes, the detected source is node $0$, the infected leaf node. However, when the number of infected nodes increases to 4 or 5, the detected source shifts to node $1$, which lies on the path from the leaf node to the central node of the rumor graph. We can also observe the same phenomenon in Fig. \ref{fig:ML_star_graph_B3-311-111}.



%{
%\captionsetup[subfigure]{skip=-0pt,position=bottom,belowskip=0pt}
%\begin{figure}[ht]
%\centering
%  \subcaptionbox{\label{fig:ML_line_graph_one_leaf_infected-3-01}}[.48\linewidth]{\includegraphics[trim={0 0 0 0em},clip,width=1.0\linewidth]{figs/ML_line_graph_one_leaf_infected-3-01.png}} \hfill
%  \subcaptionbox{\label{fig:ML_line_graph_one_leaf_infected-4-01}}[.48\linewidth]{\includegraphics[trim={0 0 0 0em},clip,width=1.0\linewidth]{figs/ML_line_graph_one_leaf_infected-4-01.png}}
%  \caption{$P(G_\text{N}|v, T)$ given by starlike tree approximation in line graphs where $G_\text{N}$ contains exactly one leaf of $G$. The estimated sources are indicated by arrows.}
%  \label{fig:line-graph-leaf-infected}
%\end{figure}
%}



{
\captionsetup[subfigure]{skip=-0pt,position=bottom,belowskip=0pt}
\begin{figure*}[ht]
\centering
  \subcaptionbox{Line graph with $3$ infected nodes.\label{fig:ML_line_graph_one_leaf_infected-3-01}}[.33\linewidth]{\includegraphics[trim={0 0 0 0em},clip,width=0.98\linewidth]{figs/ML_line_graph_one_leaf_infected-3-01.png}}\hfill
  \subcaptionbox{Line graph with $4$ infected nodes. \label{fig:ML_line_graph_one_leaf_infected-4-01}}[.33\linewidth]{\includegraphics[trim={0 0 0 0em},clip,width=0.98\linewidth]{figs/ML_line_graph_one_leaf_infected-4-01.png}}\hfill
  \subcaptionbox{Line graph with $5$ infected nodes. \label{fig:ML_line_graph_one_leaf_infected-5-01}}[.33\linewidth]{\includegraphics[trim={0 0 0 0em},clip,width=0.98\linewidth]{figs/ML_line_graph_one_leaf_infected-5-01.png}}\hfill
  \caption{$P(G_\text{N}|v, T)$ given by starlike tree approximation in line graphs where $G_\text{N}$ contains exactly one leaf of $G$. The estimated sources are indicated by arrows.}
  \label{fig:line-graph-leaf-infected}
\end{figure*}
}




\figref{fig:ML_star_graph_B3} provides an example of a starlike graph with three arms with difference lengths connected to the central node. These figures also include a curve representing $P(G_{\text{N}}|v, T)$ as a function of $T$ for a selected node $v$. In \figref{fig:ML_star_graph_B3-111-111}, the central node $0$ is identified as the estimated source as shown in Theorem~\ref{thm:central-is-source}.

In starlike tree graphs where $G_N$ does not contain any leaf node of $G$, the central node may not always be the estimated source. For example, \figref{fig:ML_star_graph_B3-311-111} is more unbalanced than \figref{fig:ML_star_graph_B3-211-111} regarding the size of the linear graphs attached to the central node. Consequently, the estimated source shifts from the central node $0$ to the non-central node $1$ in \figref{fig:ML_star_graph_B3-311-111}. Furthermore, in starlike tree graphs, when $G_N$ includes the leaf of $G$, the estimated source may shift due to the boundary effect~\cite{pd_ASONAM}. For example, the estimated source is node $4$ in \figref{fig:ML_star_graph_B3-311-011}, which differs from that in \figref{fig:ML_star_graph_B3-311-111}. 




{
\captionsetup[subfigure]{skip=-0pt,position=bottom,belowskip=0pt}
\begin{figure}[ht]
\centering
  \subcaptionbox{\label{fig:ML_star_graph_B3-111-111}}[.48\linewidth]{\includegraphics[trim={0 0 0 0em},clip,width=1.05\linewidth]{figs/ML_star_graph_B3-111-111.png}} \hfill
  \subcaptionbox{\label{fig:ML_star_graph_B3-211-111}}[.48\linewidth]{\includegraphics[trim={0 0 0 0em},clip,width=1.05\linewidth]{figs/ML_star_graph_B3-211-111.png}}\\
  \subcaptionbox{\label{fig:ML_star_graph_B3-311-111}}[.48\linewidth]{\includegraphics[trim={0 0 0 0em},clip,width=1.05\linewidth]{figs/ML_star_graph_B3-311-111.png}} \hfill
  \subcaptionbox{\label{fig:ML_star_graph_B3-311-011}}[.48\linewidth]{\includegraphics[trim={0 0 0 0em},clip,width=1.05\linewidth]{figs/ML_star_graph_B3-311-011.png}}
  \caption{$\Tilde{P}(G_\text{N}|v, T)$ in star/starlike tree graphs where the central node has 3 infected neighbors. The estimated sources are indicated by arrows.}
  \label{fig:ML_star_graph_B3}
\end{figure}
}

\iffalse
{
\captionsetup[subfigure]{skip=-0pt,position=bottom,belowskip=0pt}
\begin{figure}[ht]
\centering
  \subcaptionbox{\label{fig:ML_star_graph_B4-1111-1111}}[.48\linewidth]{\includegraphics[trim={0 0 0 0em},clip,width=1.05\linewidth]{figs/ML_star_graph_B4-1111-1111.png}} \hfill
  \subcaptionbox{\label{fig:ML_star_graph_B4-2111-1111}}[.48\linewidth]{\includegraphics[trim={0 0 0 0em},clip,width=1.05\linewidth]{figs/ML_star_graph_B4-2111-1111.png}}\\
  \subcaptionbox{\label{fig:ML_star_graph_B4-3111-1111}}[.48\linewidth]{\includegraphics[trim={0 0 0 0em},clip,width=1.05\linewidth]{figs/ML_star_graph_B4-3111-1111.png}} \hfill
  \subcaptionbox{\label{fig:ML_star_graph_B4-3111-0111}}[.48\linewidth]{\includegraphics[trim={0 0 0 0em},clip,width=1.05\linewidth]{figs/ML_star_graph_B4-3111-0111.png}}\\
  \subcaptionbox{\label{fig:ML_star_graph_B4-4111-1111}}[.48\linewidth]{\includegraphics[trim={0 0 0 0em},clip,width=1.05\linewidth]{figs/ML_star_graph_B4-4111-1111.png}} \hfill
  \subcaptionbox{\label{fig:ML_star_graph_B4-4111-0111}}[.48\linewidth]{\includegraphics[trim={0 0 0 0em},clip,width=1.05\linewidth]{figs/ML_star_graph_B4-4111-0111.png}}\\
  \caption{$\Tilde{P}(G_\text{N}|v, T)$ in star/starlike tree graphs where the central node has 4 infected neighbors. The estimated sources are indicated by arrows.}
  \label{fig:ML_star_graph_B4}
\end{figure}
}
\fi




% {
% \captionsetup[subfigure]{skip=-0pt,position=bottom,belowskip=0pt}
% \begin{figure*}[ht]
% \centering
%   \subcaptionbox{Star graph with $4$ infected nodes. The curves for nodes $2$ and $3$ are overlapping with that for node $1$, hence omitted.\label{fig:ML_star_graph-with_network_N4}}[.48\linewidth]{\includegraphics[trim={0 0 0 0em},clip,width=0.75\linewidth]{figs/ML_star_graph-with_network_N4.png}} \hfill
%   \subcaptionbox{Star graph with $5$ infected nodes. The curves for nodes $2, 3$, and $4$ are overlapping with that for node $1$, hence omitted. \label{fig:ML_star_graph-with_network_N5}}[.48\linewidth]{\includegraphics[trim={0 0 0 0em},clip,width=0.75\linewidth]{figs/ML_star_graph-with_network_N5.png}}\hfill
%   \caption{$P(G_\text{N}|v, T)$ given by our proposed method in star graphs. The center node is the detected rumor source.}
%   \label{fig:ML_star_graph-with_network}
% \end{figure*}
% }



\subsection{Comparison with existing methods}
% ~\figref{fig:customized_G} shows a grid graph with the estimated source by starlike tree approximation and typical methods indicated. In this grid graph, the estimated source given by starlike tree approximation is different from that given by rumor centrality with BFS heuristic.


% To evaluate the performance of starlike tree approximation and compare it with typical existing methods, simulation results are carried out on Random Tree, Erdős–Rényi model, and Watts–Strogatz model~\cite{watts1998collective}. Random Tree generates a tree that is uniformly chosen from the set of all trees on the given nodes, and the latter two models generates general graphs. For all the models, the underlying networks with a number of $n\in \{50, 100, 150, 200, 250, 300\}$ nodes are generated. For Erdős–Rényi model, the probability for there being edges between a pair of nodes is chosen to be $0.04$; and for Watts–Strogatz model, each node is joined with its $\ceil*{0.04n}+1$ neighbors in a ring topology and the probability for rewiring each edge is $0.1$, where $\ceil{x}$ means the least integer greater than or equal to $x$.

%To assess the performance of the starlike tree approximation and compare it with existing methods, we conducted simulation experiments on the Random Tree, Erdős–Rényi model, and Watts–Strogatz model \cite{watts1998collective}. Random Tree generates a tree selected uniformly from the set of all possible trees with the given number of nodes, while the latter two models generate general graphs. In all models, we generated underlying networks with varying numbers of nodes, specifically $n\in \{50, 100, 150, 200, 250, 300\}$. For the Erdős–Rényi model, we set the probability of having edges between any pair of nodes to be $0.04$. In the Watts–Strogatz model, each node is connected to its $\ceil*{0.04n}+1$ neighbors in a ring topology, and the probability of rewiring each edge is $0.1$. Here, $\ceil{x}$ denotes the smallest integer greater than or equal to $x$.

%short_Version
%--------------------------
\subsubsection{Synthetic Data}
To assess the performance of the starlike tree approximation and compare it with existing methods, we conducted simulation experiments on the Random Trees and Erdős–Rényi (ER) random graphs. Random Tree generates a tree selected uniformly from the set of all possible trees with the given number of nodes, while the latter two models generate general graphs. In all models, we generated underlying networks with varying numbers of nodes, specifically $n\in \{50, 100, 150, 200, 250, 300\}$. For ER random graphs, we set the probability of having edges between any pair of nodes to be $0.04$. 



To model the rumor-spreading process, we begin by randomly selecting a node as the original source of the rumor, denoted by $v^\star$, in each generated network. The rumor propagation over time $T$ follows the model detailed in Section~\ref{sec:model}. Our analysis aims to evaluate the starlike tree approximation's accuracy against existing methods by examining various infection ratios, specifically $0.1, 0.2, 0.3, 0.4, 0.5$, and $0.6$. The comparison includes methodologies such as rumor centrality with a Breadth-First Search (BFS) heuristic, distance centrality, and the Jordan center. In instances of multiple nodes computed as the source, one is chosen at random to be the detected source.


The accuracy of rumor source detection is depicted in \figref{fig:accuracy-infection_proportion}. Overall, as the infection proportion increases, the accuracy of all methods tends to decrease. 


\begin{figure*}[ht]
\centering
  \includegraphics[width=0.98\linewidth]{figs/accuracy-infection_proportion-ER.png}
    \caption{Accuracy of the rumor detection methods against the infection proportion in Erdős–Rényi model.}
    \label{fig:accuracy-infection_proportion}
\end{figure*}





%------------------------------Full_Page_Figure- Here-------------
\iffalse
{
\captionsetup[subfigure]{skip=-0pt,position=bottom,belowskip=0pt}
\begin{figure*}[h]
\setlength{\belowcaptionskip}{0pt} 
\centering
\subcaptionbox{Random Tree.\label{fig:Accuracy_RT}}[0.98\linewidth][c]{\includegraphics[trim={0 0 0 0em},clip,width=0.8\linewidth]{figs/Accuracy_RT_with_legend.png}}\hfill 
\subcaptionbox{Erdős–Rényi model.\label{fig:Accuracy_ER}}[0.98\linewidth][c]{\includegraphics[trim={0 0 0 0em},clip,width=0.8\linewidth]{figs/Accuracy_ER.png}}\hfill \\
\subcaptionbox{Watts–Strogatz model. \label{fig:Accuracy_WSs}}[0.98\linewidth][c]{\includegraphics[trim={0 0 0 0em},clip,width=0.8\linewidth]{figs/Accuracy_WSs.png}}\hfill 
\caption{Accuracy of rumor detection methods against the number of nodes $n$ with different infection proportions in different models.}
\label{fig:accuracy-n}
\end{figure*}
}
\fi
 
%------------------------------Full_Page_Figure--------------

\begin{figure*}[ht]
\centering
  \includegraphics[scale =0.65]{figs/Accuracy_RT_with_legend2.png}
    \caption{Accuracy of the rumor detection methods against the infection proportion in random tree graphs.}
    \label{fig:Accuracy_RT}
\end{figure*}


In the case of random trees, the starlike tree approximation demonstrates higher accuracy compared to other methods when the infection proportion ranges between 0.2 and 0.3, and the number of nodes varies from 50 to 300. This superiority can be attributed to the starlike tree approximation's utilization of information from the boundary of the rumor graph, its consideration of the phase-type distribution of spreading, and its resistance to the boundary effect, in contrast to the rumor centrality with the BFS heuristic method. Given these characteristics, it is not surprising that the starlike tree approximation outperforms other methods in the Random Tree scenario, particularly when the number of nodes and the infection proportion is around $0.3$ and $0.4$.


% In fact, in degree-regular trees, rumor centrality is the ML estimator and is shown to perform well~\cite{shah2011rumors}. The underlying networks of $m$-ary Tree generated in the experiments are similar to degree-regular trees since most of the non-leaf nodes have the same degree for a given number of nodes, but there are boundary leaf nodes whose degree is only one. As a result, on one hand, rumor centrality with BFS still performs well compared to other methods when the number of nodes increases, due to the similarity between $m$-ary trees and degree-regular trees; on the other hand, there can be leaf nodes in the underlying network being infected, which lead to lower accuracy compared with that reported in degree-regular tree networks~\cite{shah2011rumors}. 


\begin{figure*}[ht]
\centering
  \includegraphics[scale =0.67]{figs/Accuracy_ER_with_legend.png}
    \caption{Accuracy of the rumor detection methods against the infection proportion in Erdős–Rényi model.}
    \label{fig:Accuracy_ER}
\end{figure*}

%In the Erdős–Rényi model and Watts–Strogatz model, as depicted in \figref{fig:Accuracy_ER} and \figref{fig:Accuracy_WSs} respectively, the starlike tree approximation demonstrates comparable accuracy across various combinations of the number of nodes and infection proportion. Notably, in the Erdős–Rényi model, the starlike tree approximation exhibits improved accuracy when the infection proportion is 0.5, and the number of nodes in the underlying network ranges from 50 to 250.

In the Erdős–Rényi model, as depicted in \figref{fig:Accuracy_ER}, the starlike tree approximation demonstrates comparable accuracy across various combinations of the number of nodes and infection proportion. Notably, in the Erdős–Rényi model, the starlike tree approximation exhibits improved accuracy when the infection proportion is 0.5, and the number of nodes in the underlying network ranges from 50 to 250.

%\begin{figure*}[ht]
%\centering
%  \includegraphics[scale =0.65]{figs/Accuracy_WSs_legend.png}
%    \caption{Accuracy of the rumor detection methods against the infection proportion in Watts–Strogatz model.}
%    \label{fig:Accuracy_WSs}
%\end{figure*}

\subsubsection{Real World Networks}

Based on our experiments, the starlike tree approximation appears to be preferred for the accurate detection of rumor sources in the Random Tree, and Erdős–Rényi model, particularly when dealing with a moderate number of nodes and infection ratio. The source code of the above simulation can be publicly accessed at \url{https://github.com/convexsoft/Rumor-Source-Detection}.



% While for the networks resembling the degree-regular tree, e.g., $m$-ary tree, our method is inferior to the rumor centrality with BFS heuristic method.






